On the Characterization of Local Nash Equilibria in Continuous Games

We present a unified framework for characterizing local Nash equilibria in continuous games on either infinite-dimensional or finite-dimensional non-convex strategy spaces. We provide intrinsic necessary and sufficient first- and second-order conditions ensuring strategies constitute local Nash equilibria. We term points satisfying the sufficient conditions differential Nash equilibria. Further, we provide a sufficient condition (non-degeneracy) guaranteeing differential Nash equilibria are isolated and show that such equilibria are structurally stable. We present tutorial examples to illustrate our results and highlight degeneracies that can arise in continuous games.

==> makefile <==
# set latexfile to the name of the main file without the .tex
latexfile = 2014IEEETACv1s
# put the names of figure files here.  include the .eps
#figures = 
# if no references, run "touch latexfile.bbl; touch referencefile.bib"
# or delete dependency in .dvi and tarball sections
# referencefile = poster


TEX = pdflatex

# support subdirectories
VPATH = Figs

$(latexfile).pdf : $(figures) $(latexfile).tex 
#$(latexfile).dvi : $(figures) $(latexfile).tex $(latexfile).bbl
	while ($(TEX) $(latexfile) ; \
	grep -q "Rerun to get cross" $(latexfile).log ) do true ; \
	done


$(latexfile).tar.gz : $(figures) $(latexfile).tex
	tar -czvf $(latexfile).tar.gz $^

tarball: $(latexfile).tar.gz

cpall:
	make; skim $(latexfile).pdf

bib:
	bibtex $(latexfile)

clean:
	rm $(latexfile).dvi $(latexfile).log $(latexfile).ps $(latexfile).pdf

mpdf:
	pdflatex $(latexfile).tex; skim $(latexfile).pdf

